Interaction-aware Model Predictive Control for Autonomous Driving

Lane changing and lane merging remains a challenging task for autonomous driving, due to the strong interaction between the controlled vehicle and the uncertain behavior of the surrounding traffic participants. The interaction induces a dependence of the vehicles' states on the (stochastic) dynamics of the surrounding vehicles, increasing the difficulty of predicting future trajectories. Furthermore, the small relative distances cause traditional robust approaches to become overly conservative, necessitating control methods that are explicitly aware of inter-vehicle interaction. Towards these goals, we propose an interaction-aware stochastic model predictive control (MPC) strategy integrated with an online learning framework, which models a given driver's cooperation level as an unknown parameter in a state-dependent probability distribution. The online learning framework adaptively estimates the surrounding vehicle's cooperation level with the vehicle's past trajectory and combines this with a kinematic vehicle model to predict the probability of a multimodal future state trajectory. The learning is conducted with logistic regression which enables fast online computation. The multi-future prediction is used in the MPC algorithm to compute the optimal control input while satisfying safety constraints. We demonstrate our algorithm in an interactive lane changing scenario with drivers in different randomly selected cooperation levels.

==> content/algorithm.tex <==
% For each mode $w_i$ and input sequence $\boldsymbol{u}^{(w_i), \tv}$, a trajectory is predicted. Accordingly, optimal control inputs are computed for each trajectory individually with constraint that each control sequence share the same first component. The reason for adoption of multiple control sequences formulation is to avoid conservatism as stated in \cite{nair2022stochastic}. the optimal control problem is written as: \textcolor{red}{Any suggestion on layout \eqref{eq: objective}?}
% \begin{subequations}\label{eq: final_form}
% \begin{align}
% 	\min_{u^\ego_0}\quad &  \ell(z_0^\ego, u_0^\ego \;;\; z_0^{ref, \ego})\label{eq: objective}\\
% + {} \sum_{w_i}\hat{p}_{w_i}(\bar{z}_0^\ego, \bar{z}_0^\tv) \Big(\min_{u^{w_i, \ego}_1, \dots} \; & \sum_{k = 1}^{N-1} \ell(z_k^{{w_i}, \ego}, u_k^{{w_i}, \ego}) + \ell_N(z_N^{{w_i}, \ego})\Big)\notag \\
% 	\text{s.t.} \quad z_0^{w_i, \ego} &= \bar{z}_0^\ego \\
% 	z_0^{w_i, \tv} &= \bar{z}_0^\tv \\
% 	 z^{{w_i}, \ego}_{k+1} &= f\big(z^{{w_i}, \ego}_k, u_k^{w_i, \ego}\big)\\
% z^{{w_i}, \tv}_{k+1} &= f(z^{{w_i}, \tv}_k, u_k^{w_i, \tv}) \\
% \sum_{w_i}\hat{p}_{w_i}\sigma\Big(\big(\text{dist}(O_{k, i}^{w_i, \ego}, O_{k, j}^{w_i, \tv}) & \leq 4r^2\big)\Big)  \leq \gamma,\quad  k \leq 2\\
% \big(\text{dist}\big((O_{i, k}^{w_i, \ego}, O_{j, k}^{w_i, \tv})\big)^2 &\geq 4r^2, \quad k>2\\
% u_k^{w_i, \ego} &\in \mathcal{U} \\
% \Delta u_k^{w_i, \ego} & \in \Delta\mathcal{U} \\
% z_k^{w_i, \ego} &\in \mathcal{Z}
% \end{align}
% \end{subequations}

% The full algorithm is summarized below:
% \begin{algorithm}
% \caption{Interaction-aware MPC}\label{alg: int-mpc}
% \begin{algorithmic}
%     \Initialize{Measurement $\bar{z}^\ego_0$, $\bar{z}^\tv_0$, parameter $\param_0$}
%     \For{$\tau=1, 2, 3 \dots$}
%     \State Compute probability $\hat{P}(\bar{z}^\ego_{\tau-1}, \bar{z}^\tv_{\tau-1})$
%     \State Solve \cref{eq: final_form} to obtain the optimal control inputs $\boldsymbol{u}^*$
%     \State Apply $u_\tau^* = \boldsymbol{u}^*(0)$ to the system
%     \State Measure states $\bar{z}^\ego_\tau, \bar{z}^\tv_\tau$
%     \State Update parameter $\param_\tau$ using \cref{eq: param_update}
%     \EndFor
% \end{algorithmic}
% \end{algorithm}

==> content/symbol_list.tex <==
\begin{supertabular*}{\textwidth}{ll}
\multicolumn{2}{l}{\bf \Large Latin letters} \\
\\
\hline 
{\bf Symbol}					&		{\bf Meaning} \\
\hline
\\
a                               &  acceleration \\
$h(z^e, z^t)$                   &  feature function \\
k                               &  time step in prediction \\
$M$                             &  weights for terminal cost \\
$n$                             & total number of datapoints collected online \\
$n_c$                           &  number of circles \\
$n_m$                               &  number of modes \\
N                               & prediction horizon \\
$N_d$                             & number of datapoints\\
$p_i$                           &  probability of mode i \\
$P$                           &  distribution of choosing modes \\
Q                               &  weights for states \\
$r_c$                               &  radius of circles in collision avoidance constraints \\
R                               &  weights for input  \\
t                               &  time step in simulation \\
$T_s$                           & sampling time \\
$\Delta u_k$                    &  input difference at time step k ($\Delta u_k = u_{k+1} - u_k$)\\
$u^{(i)}(\cdot)$                &  closed-loop control law in mode i \\
$u^{\{e, t\}}_k$                 &  ego / target vehicle's input at time step k \\
$U(a, b)$                       & uniform distribution from a to b \\
$w$                             & random variable to denote mode \\
$v$                             &  speed in all direction \\
$V$                             &  value function \\
$\pos_x$                             &  coordinate of the center of gravity\\
$y_i$                           &  label of $i$th datapoint \\
$\pos_y$                             &  coordinate of the center of gravity\\
$z^{\{e, t\}}_k$                  &  ego / target vehicle's states at time step k \\
\\
\\
\\
\multicolumn{2}{l}{\bf \Large Greek letters} \\
\\
\hline 
{\bf Symbol}					&		{\bf Meaning} \\
\hline
$\alpha_0, \alpha_1$            & intercept and weights to approximate step function $\mathbbm{1}$ \\
$\beta$                         &  slip angle of the center of gravity \\
$\beta_{i0}, \boldsymbol{\beta}_i$ & intercept and weights for mode i \\
$\steer$                      &  steering angle \\ 
$\gamma$                        & threshold in \eqref{eq: collision_avoidance_chance} \\
$\psi$                          &  heading \\
$\param$                        &  parameter in distribution \\
$\lambda$                       & weights for regularization \\
$\sigma$                        & sigmoid function
$\tau$                          & time step in the simulation\\
\\
\\
\\
\\
\multicolumn{2}{l}{\bf \Large Calligraphic and other symbols} \\
\\
\hline 
{\bf Symbol}					&		{\bf Meaning} \\
\hline
\\
$\mathcal{U}$                   & set of input constraints \\
$\Delta\mathcal{U}$             & set of input difference constraints \\
$\mathcal{Z}$                   & set of states constraints \\
\\
\\
\\

\end{supertabular*}

\cleardoublepage

==> tikz/autodriving.tex <==
        % ========================================
        % DEFINE COLORS 
        % ========================================

        \definecolor{roadborder}{HTML}{97adc6}
        \definecolor{road}{HTML}{65758e}
        \definecolor{stripes}{rgb}{1,1,1}
        % \definecolor{grass}{HTML}{bced9c}
        \definecolor{leaf}{HTML}{bced9c}  % Forestgreen
        % \definecolor{leaf}{HTML}{32CD32}    % Lime green
        % \definecolor{leaf}{HTML}{00A36C}    % Jade
        \definecolor{windshield}{HTML}{cfe3f9}
        \definecolor{car1color}{HTML}{267de0}
        \definecolor{car2color}{HTML}{e04825}
        \definecolor{car3color}{HTML}{FF4422}

        \definecolor{darkblue}{HTML}{185973}
        \colorlet{learningColor}{darkblue}
        \definecolor{fwoColor}{rgb}{0.85, 0.85, 0.85}

        % ========================================
        % DEFINE ROAD SEGMENTS AND CARS
        % ========================================
        \tikzset{
            pics/pedestrian/.style args={#1}{code={
                \def\shoulderwidth{2}
                \def\thickness{0.5}
                \fill[fill=#1, rounded corners] ({-0.5*\thickness}, {-0.5*\shoulderwidth}) rectangle ({0.5*\thickness}, {0.5*\shoulderwidth});
                \draw[fill=black, draw=none] (0,0) circle ({0.2*\shoulderwidth});
            }},
            pics/bicycle/.style args={#1}{code={
                \def\bikelength{4.5}
                \def\bikewidth{0.3}
                \fill[fill=black!80, rounded corners] (0, {-0.5*\bikewidth}) rectangle ({0.3*\bikelength}, {0.5*\bikewidth});
                \fill[fill=black!80, rounded corners] ({0.5*\bikelength}, {-0.5*\bikewidth}) rectangle ({\bikelength}, {0.5*\bikewidth});
                \fill[fill=black!70, rounded corners] ({0.5*\bikelength}, {-\bikewidth}) rectangle ({0.85*\bikelength}, {\bikewidth});

                % \fill[fill=#1, rounded corners] (0, {-0.5*\bikewidth}) rectangle ({\bikelength}, {0.5*\bikewidth});
                % \fill[rounded corners]
                \fill[fill=black!10, rounded corners] ({0.27*\bikelength}, {3*\bikewidth}) rectangle ({0.31*\bikelength}, {-3*\bikewidth});
                \fill[fill=black!10, rounded corners] ({0.27*\bikelength}, {3*\bikewidth}) rectangle ({0.31*\bikelength}, {-3*\bikewidth});

                \fill[fill=#1] ({0.43*\bikelength}, {3.3*\bikewidth}) arc (90:-90:{3.3*\bikewidth});
                \draw[fill=black, line width=0.35cm, rounded corners] ({0.44*\bikelength}, {2.6*\bikewidth}) -- ({0.27*\bikelength}, {3*\bikewidth});
                \draw[fill=black, line width=0.35cm, rounded corners] ({0.44*\bikelength}, {-2.6*\bikewidth}) -- ({0.27*\bikelength}, {-3*\bikewidth});

                \draw[fill=black, draw=none] ({0.4*\bikelength},0) circle ({0.1*\bikelength});
            }},
            pics/road/.style n args={4}{code={
                \def\roadW{#1}
                \def\roadL{#2}
                \def\lineL{2}
                \pgfmathsetmacro\nLines{int(floor(\roadL/\lineL))}
                % \def\nLines{}
                \fill[fill=road] (0,{-0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW}); 
                \foreach \i in {0,...,{\nLines}}
                {   
                    \fill[fill=stripes] ({\i*\lineL}, {-0.01*\roadW}) rectangle ({(\i+0.8)*\lineL}, {0.01*\roadW});
                }
                
                \fill[fill=roadborder] (0, {0.5*\roadW}) rectangle ({\roadL}, {0.5*\roadW+2}); 
                \fill[fill=roadborder] (0, {-0.5*\roadW}) rectangle ({\roadL}, {-0.5*\roadW-2});

                \ifthenelse {\isempty{#4}}{}
                        {\fill[fill=stripes] (0.0*\roadW,{0.0*\roadW}) rectangle ({0.05*\roadW}, {0.45*\roadW});
                        }                       
            }},
            pics/roadblock/.style n args={4}{code={
                \def\roadW{#1}
                \def\roadL{#2}
                \def\lineL{2}
                \def\block{#3}
                \def\smoothblockL{8}
                \def\overlap{0.05}
                \pgfmathsetmacro\nLines{int(floor((\block-0.05)*\roadL/\lineL))}
                % \def\nLines{}

                \fill[fill=roadborder] (0, {0.5*\roadW}) rectangle ({\block*\roadL}, {0.5*\roadW+2}); 
                \fill[fill=roadborder] ({\block*\roadL + \smoothblockL}, 0) rectangle ({\roadL}, 2);
                \fill [fill = roadborder, domain=-5:8, variable=\x]
                (\block*\roadL-\overlap, -\overlap)
                -- plot ({\block*\roadL + 5 + \x}, {2+((0.505)*\roadW)*(1-1/(1+e^(-\x)))})
                -- (\block*\roadL + 13, -\overlap)
                -- cycle;
                \fill[fill=roadborder] (0, {-0.5*\roadW}) rectangle ({\roadL}, {-0.5*\roadW-2});

                \fill[fill=road] (0,-\overlap) rectangle ({\block*\roadL+\overlap}, {0.5*\roadW});
                \fill[fill=road] (0,{-0.5*\roadW}) rectangle ({\roadL}, 0);

                \fill [fill = road, domain=-4:8, variable=\x]
                (\block*\roadL-\overlap, -\overlap)
                -- plot ({\block*\roadL + 4 + \x}, {((0.51)*\roadW)*(1-1/(1+e^(-\x)))})
                -- (\block*\roadL + 12, -\overlap)
                -- cycle;

                \foreach \i in {0,...,{\nLines}}
                {   
                    \fill[fill=stripes] ({\i*\lineL}, {-0.01*\roadW}) rectangle ({(\i+0.8)*\lineL}, {0.01*\roadW});
                }
                

                \ifthenelse {\isempty{#4}}{}
                        {\fill[fill=stripes] (0.0*\roadW,{0.0*\roadW}) rectangle ({0.05*\roadW}, {0.45*\roadW});
                        }                       
            }},
            pics/roadblock2/.style n args={4}{code={
                \def\roadW{#1}
                \def\roadL{#2}
                \def\lineL{2}
                \def\block{#3}
                \def\smoothblockL{8}
                \def\overlap{0.05}
                \pgfmathsetmacro\nLines{int(floor((\block-0.05)*\roadL/\lineL))}
                % \def\nLines{}

                \fill[fill=roadborder] (0, {0.5*\roadW}) rectangle ({\block*\roadL}, {0.5*\roadW+1}); 
                \fill[fill=roadborder] ({\block*\roadL + \smoothblockL}, 0) rectangle ({\roadL}, 1);
                \fill [fill = roadborder, domain=-5:8, variable=\x]
                (\block*\roadL-\overlap, -\overlap)
                -- plot ({\block*\roadL + 4.5 + \x}, {1+((0.505)*\roadW)*(1-1/(1+e^(-\x)))})
                -- (\block*\roadL + 12.5, -\overlap)
                -- cycle;
                \fill[fill=roadborder] (0, {-0.5*\roadW}) rectangle ({\roadL}, {-0.5*\roadW-1});

                \fill[fill=road] (0,-\overlap) rectangle ({\block*\roadL+\overlap}, {0.5*\roadW});
                \fill[fill=road] (0,{-0.5*\roadW}) rectangle ({\roadL}, 0);

                \fill [fill = road, domain=-4:8, variable=\x]
                (\block*\roadL-\overlap, -\overlap)
                -- plot ({\block*\roadL + 4 + \x}, {((0.51)*\roadW)*(1-1/(1+e^(-\x)))})
                -- (\block*\roadL + 12, -\overlap)
                -- cycle;

                \foreach \i in {0,...,{\nLines}}
                {   
                    \fill[fill=stripes] ({\i*\lineL}, {-0.01*\roadW}) rectangle ({(\i+0.8)*\lineL}, {0.01*\roadW});
                }
                

                \ifthenelse {\isempty{#4}}{}
                        {\fill[fill=stripes] (0.0*\roadW,{0.0*\roadW}) rectangle ({0.05*\roadW}, {0.45*\roadW});
                        }                       
            }},
            pics/car/.style args={#1}{
            code={
            \def\carw{3}
            \def\carh{6.5}
            \def\winmarginx{0.2}
            \def\wintiltinward{0.2}
            \def\winradiusfront{7}
            \def\winradiusback{10}
            \def\winmarginy{2}
            \def\winh{1}
            \def\alphafront{30}
            \def\alphaback{120}
            
            % \draw [help lines, #1!10] (0,0) grid (\carw, \carh);
            \fill[fill=#1, rounded corners=20] (\carw,0) -- ++(0, \carh) -- ++(-\carw, 0) [rounded corners=30] -- ++(0, -\carh) -- cycle;

            %--------------------
            % Front windshield 
            %--------------------
            \def\centerY{7}
            \def\rad{\centerY-\winmarginy}
            \def\theta{15} 
            \def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
            \def\ytop{\centerY - (\rad)*cos(\theta)}

            \def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
            \def\ybot{\centerY - (\rad-\winh)*cos(\theta)}

            \def\startalpha{270+\theta}
            \def\endalpha{270-\theta}

            \fill[fill=windshield, ] ({\xtop}, {\ytop}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});
            
            %--------------------
            % Back windshield 
            %--------------------

            \def\winmarginy{0.7}
            \def\centerY{\carw-8}
            \def\winh{0.5}
            \def\theta{18} 
            \def\rad{\carw+\centerY-\winmarginy}
            \def\xtop{0.5*(\carw) + (\rad)*sin(\theta)}
            \def\ytopback{\carw- (\centerY - (\rad)*cos(\theta))}

            \def\xbot{0.5*(\carw) - (\rad-\winh)*sin(\theta)}
            \def\ybot{\carw- (\centerY - (\rad-\winh)*cos(\theta))}

            \def\startalpha{270+\theta}
            \def\endalpha{270-\theta}

            \fill[fill=windshield] ({\xtop}, {\ytopback}) arc({\startalpha}:{\endalpha}:{\rad}) -- ({\xbot}, {\ybot}) arc({\endalpha}:{\startalpha}:{\rad-\winh});

            %--------------------
            % left window 
            %--------------------

            \def\centerleft{-4}
            \def\marginx{0.2}
            \def\radius{\marginx-\centerleft}
            \def\angle{20}
            \def\top{0.5*\carh + (\radius)*sin(\angle)}
            \def\bottom{0.5*\carh - (\radius)*sin(\angle)}

            \fill[fill=windshield, ] ({\marginx}, {\top}) arc(0.5*\angle: -0.5*\angle: {\radius}) -- cycle;
            \fill[fill=windshield, ] ({\carw-\marginx}, {\top}) arc(180-0.5*\angle: 180+0.5*\angle: {\radius}) -- cycle;
            arc({\endalpha}:{\startalpha}:{\rad-\winh});

            % ----------------------------
            % Left mirror 
            % ----------------------------
            \def\mirrorY{0.4*\carh}
            \fill[fill=#1] ({0.05*\carw}, {\mirrorY}) arc(0:-180:0.3) -- cycle;
            \fill[fill=#1] ({0.95*\carw}, {\mirrorY}) arc(-180:0:0.3) -- cycle;
            }
            }
        }
